Merging multiple input descriptors and supervisors in a deep neural network for tractogram filtering

One of the main issues of the current tractography methods is their high false-positive rate. Tractogram filtering is an option to remove false-positive streamlines from tractography data in a post-processing step. In this paper, we train a deep neural network for filtering tractography data in which every streamline of a tractogram is classified as {\em plausible, implausible}, or {\em inconclusive}. For this, we use four different tractogram filtering strategies as supervisors: TractQuerier, RecobundlesX, TractSeg, and an anatomy-inspired filter. Their outputs are combined to obtain the classification labels for the streamlines. We assessed the importance of different types of information along the streamlines for performing this classification task, including the coordinates of the streamlines, diffusion data, landmarks, T1-weighted information, and a brain parcellation. We found that the streamline coordinates are the most relevant followed by the diffusion data in this particular classification task.

==> methods/overview.tex <==

\newlength{\w}
\setlength{\w}{6mm}

\newlength{\hxyz}
\setlength{\hxyz}{4mm}
\newlength{\hlm}
\setlength{\hlm}{7mm}
\newlength{\htone}
\setlength{\htone}{3mm}
\newlength{\hsh}
\setlength{\hsh}{9mm}
\newlength{\hparc}
\setlength{\hparc}{12mm}

\begin{figure}
    \centering
    \tikzset{%
        conv/.style = {node distance=3\w,rectangle, minimum height=12mm, draw},
        conv_fill/.style = {node distance=2\w},
        merged/.style = {rectangle, minimum height=2mm},
        layer_1/.style = {minimum width=2\w},
        layer_2/.style = {minimum width=1.8\w},
        layer_3/.style = {minimum width=1.5\w},
        branch_xyz/.style = {draw=red},
        branch_lm/.style = {draw=green},
        branch_t1/.style = {draw=blue},
        branch_sh/.style = {draw=orange},
        branch_parc/.style = {draw=gray},
        in_xyz/.style = {minimum height=\hxyz},
        in_lm/.style = {minimum height=\hlm},
        in_t1/.style = {minimum height=\htone},
        in_sh/.style = {minimum height=\hsh},
        in_parc/.style = {minimum height=\hparc}
    }
    \begin{tikzpicture}
        % nodes of input branches
        \draw
            node[conv, branch_xyz, layer_1, in_xyz] (a1) {\tiny xyz}
            node[conv, branch_xyz, layer_2, right of=a1] (b1) {\tiny Conv}
            node[conv_fill, right of=b1] (c1) {$\cdots$}
            node[conv, conv_fill, branch_xyz, layer_3, right of=c1] (d1) {\tiny Conv};
        \draw
            node[conv, branch_lm, layer_1, in_lm, below of=a1] (a2) {\tiny landmarks}
            node[conv, branch_lm, layer_2, right of=a2] (b2) {\tiny Conv}
            node[conv_fill, right of=b2] (c2) {$\cdots$}
            node[conv, conv_fill, branch_lm, layer_3, right of=c2] (d2) {\tiny Conv};
        \draw
            node[conv, branch_t1, layer_1, in_t1, below of=a2] (a3) {\tiny T1w}
            node[conv, branch_t1, layer_2, right of=a3] (b3) {\tiny Conv}
            node[conv_fill, right of=b3] (c3) {$\cdots$}
            node[conv, conv_fill, branch_t1, layer_3, right of=c3] (d3) {\tiny Conv};
        \draw
            node[conv, branch_sh, layer_1, in_sh, below of=a3] (a4) {\tiny SH coeffs}
            node[conv, branch_sh, layer_2, right of=a4] (b4) {\tiny Conv}
            node[conv_fill, right of=b4] (c4) {$\cdots$}
            node[conv, conv_fill, branch_sh, layer_3, right of=c4] (d4) {\tiny Conv};
        \draw
            node[conv, branch_parc, layer_1, in_parc, below of=a4] (a5) {\tiny wmparc}
            node[conv, branch_parc, layer_2, right of=a5] (b5) {\tiny Conv}
            node[conv_fill, right of=b5] (c5) {$\cdots$}
            node[conv, conv_fill, branch_parc, layer_3, right of=c5] (d5) {\tiny Conv};
        % decorations of input branches
        \draw[decorate, decoration={brace,amplitude=5pt,raise=5pt}] (a1) +(-\w,0.15) -- node[midway, above=3.5mm] {$N$} +(\w,0.15);
        \draw[decorate, decoration={brace,amplitude=2pt,raise=2pt,mirror}] (a1) +(-0.7,0.5\hxyz) -- node[midway, left=3mm] {$c_{xyz}$} +(-0.7,-0.5\hxyz);
        \draw[decorate, decoration={brace,amplitude=2pt,raise=2pt,mirror}] (a2) +(-0.7,0.5\hlm) -- node[midway, left=3mm] {$c_{lm}$} +(-0.7,-0.5\hlm);
        \draw[decorate, decoration={brace,amplitude=2pt,raise=2pt,mirror}] (a3) +(-0.7,0.5\htone) -- node[midway, left=3mm] {$c_{t1}$} +(-0.7,-0.5\htone);
        \draw[decorate, decoration={brace,amplitude=5pt,raise=5pt,mirror}] (a4) +(-0.6,0.5\hsh) -- node[midway, left=3mm] {$c_{sh}$} +(-0.6,-0.5\hsh);
        \draw[decorate, decoration={brace,amplitude=5pt,raise=5pt,mirror}] (a5) +(-0.6,0.5\hparc) -- node[midway, left=3mm] {$c_{parc}$} +(-0.6,-0.5\hparc);
        % merge operation
        \draw (d3) ++(3.4\w,0)
            node [conv, layer_3, branch_xyz, above=18mm] (e1) {}
            node [conv, layer_3, branch_lm, anchor=north west] (e2) at (e1.south west) {}
            node [conv, layer_3, branch_t1, anchor=north west] (e3) at (e2.south west) {}
            node [conv, layer_3, branch_sh, anchor=north west] (e4) at (e3.south west) {}
            node [conv, layer_3, branch_parc, anchor=north west] (e5) at (e4.south west) {};
        % connections (input)
        \draw (a1) -- (b1) -- (c1) -- (d1) -- (e1);
        \draw (a2) -- (b2) -- (c2) -- (d2) -- (e2);
        \draw (a3) -- (b3) -- (c3) -- (d3) -- (e3);
        \draw (a4) -- (b4) -- (c4) -- (d4) -- (e4);
        \draw (a5) -- (b5) -- (c5) -- (d5) -- (e5);
        % nodes of output branches
        \draw (e1.center) ++(2.5,0.3) coordinate (tmp)
            node [merged, layer_3, branch_xyz, above=4mm] (f1_top) {}
            node [merged, layer_3, branch_lm, anchor=north west] (tmp) at (f1_top.south west) {}
            node [merged, layer_3, branch_t1, anchor=north west] (f1) at (tmp.south west) {\tiny Conv}
            node [merged, layer_3, branch_sh, anchor=north west] (tmp) at (f1.south west) {}
            node [merged, layer_3, branch_parc, anchor=north west] (f1_bottom) at (tmp.south west) {};
        \draw
            (f1)
            node [conv_fill, right of=f1] (tmp) {$\cdots$}
            node [conv, node distance=\w, right of=tmp] (g1) {\tiny FC}
            node [draw, rectangle, right of=g1] (h1) {$M^\ast_{rb}$};
        \draw[node distance=3\w]
            coordinate [below of=f1] (tmp)
            node [merged, layer_3, branch_xyz, above=4mm] (f2_top) at (tmp) {}
            node [merged, layer_3, branch_lm, anchor=north west] (tmp) at (f2_top.south west) {}
            node [merged, layer_3, branch_t1, anchor=north west] (f2) at (tmp.south west) {\tiny Conv}
            node [merged, layer_3, branch_sh, anchor=north west] (tmp) at (f2.south west) {}
            node [merged, layer_3, branch_parc, anchor=north west] (f2_bottom) at (tmp.south west) {};
        \draw
            (f2)
            node [conv_fill, right of=f2] (tmp) {$\cdots$}
            node [conv, node distance=\w, right of=tmp] (g2) {\tiny FC}
            node [draw, rectangle, right of=g2] (h2) {$M^\ast_{ext}$};
        \draw[node distance=3\w]
            coordinate [below of=f2] (tmp)
            node [merged, layer_3, branch_xyz, above=4mm] (f3_top) at (tmp) {}
            node [merged, layer_3, branch_lm, anchor=north west] (tmp) at (f3_top.south west) {}
            node [merged, layer_3, branch_t1, anchor=north west] (f3) at (tmp.south west) {\tiny Conv}
            node [merged, layer_3, branch_sh, anchor=north west] (tmp) at (f3.south west) {}
            node [merged, layer_3, branch_parc, anchor=north west] (f3_bottom) at (tmp.south west) {};
        \draw
            (f3)
            node [conv_fill, right of=f3] (tmp) {$\cdots$}
            node [conv, node distance=\w, right of=tmp] (g3) {\tiny FC}
            node [draw, rectangle, right of=g3] (h3) {$M^\ast_{ts}$};
        \draw[node distance=3\w]
            coordinate [below of=f3] (tmp)
            node [merged, layer_3, branch_xyz, above=4mm] (f4_top) at (tmp) {}
            node [merged, layer_3, branch_lm, anchor=north west] (tmp) at (f4_top.south west) {}
            node [merged, layer_3, branch_t1, anchor=north west] (f4) at (tmp.south west) {\tiny Conv}
            node [merged, layer_3, branch_sh, anchor=north west] (tmp) at (f4.south west) {}
            node [merged, layer_3, branch_parc, anchor=north west] (f4_bottom) at (tmp.south west) {};
        \draw
            (f4)
            node [conv_fill, right of=f4] (tmp) {$\cdots$}
            node [conv, node distance=\w, right of=tmp] (g4) {\tiny FC}
            node [draw, rectangle, right of=g4] (h4) {$M^\ast_{tq}$};
        % connections (output)
        \draw [decorate, decoration={brace,amplitude=5pt,raise=5pt}] (e1.north east) -- node [midway, right=8mm] (concat) {} (e5.south east);
        \draw []
            coordinate (concat) at (concat)
            (concat) -- +(-5mm,0)
            (concat) |- (f1)
            (concat) |- (f2)
            (concat) |- (f3)
            (concat) |- (f4);
        % branch labels
        \draw [decorate, decoration={brace,amplitude=5pt,raise=7mm,mirror}]
            (a5.south west) -- node [midway, below=1cm] {input branches} (e5 |- a5.south west);
        \draw [decorate, decoration={brace,amplitude=5pt,raise=7mm,mirror}]
            (concat |- a5.south west) -- node [midway, below=1cm] {output branches} (h4.south east |- a5.south west);
        % merge label
        \draw [shorten <=4mm, shorten >=4mm]
            (e1) -- ++(1, 2.2)
            node {concatenate channels};
    \end{tikzpicture}
    \caption{Overview about the employed network architecture. Each input modality ('xyz', 'landmarks', 'T1w', 'SH coeffs', 'wmparc') is assigned to an individual input branch of convolutional blocks ('Conv'). The outputs of all input branches are concatenated along the channel dimension and forwarded to each output branch resulting in the respective predictions for the corresponding supervisor labels. Each input encodes information per individual streamline. The inputs are of the same length $N$ but differ in the number of channels ($c_{xyz}$, $c_{lm}$, $c_{t1}$, $c_{sh}$ and $c_{parc}$).}
    \label{fig:overview_model}
\end{figure}
